MATHWELL: Generating Educational Math Word Problems Using Teacher Annotations

Math word problems are critical K-8 educational tools, but writing them is time consuming and requires extensive expertise. To be educational, problems must be solvable, have accurate answers, and, most importantly, be educationally appropriate. We propose that language models have potential to support K-8 math education by automatically generating word problems. However, evaluating educational appropriateness is hard to quantify. We fill this gap by having teachers evaluate problems generated by LLMs, who find existing models and data often fail to be educationally appropriate. We then explore automatically generating educational word problems, ultimately using our expert annotations to finetune a 70B language model. Our model, MATHWELL, is the first K-8 word problem generator targeted at educational appropriateness. Further expert studies find MATHWELL generates problems far more solvable, accurate, and appropriate than public models. MATHWELL also matches GPT-4's problem quality while attaining more appropriate reading levels for K-8 students and avoiding generating harmful questions.

==> Generations/llema_inaccurate.tex <==
Question: Batman has 5000 Joker coins, 2000 Batman coins, and 7000 Poison Ivy coins. He wants to distribute them to three different Joker's henchmen. He gives 1/3 of his Joker coins, 2/5 of his Batman coins, and 2/3 of his Poison Ivy coins to each of the Joker's henchmen. How many Joker coins does each Joker's henchman get? 

Solution: 
def solution(): 
     \indent \#Batman has 5000 Joker coins 
     \indent joker\_coins\_total = 5000 
     \indent \#Batman gives 1/3 of his Joker coins 
     \indent joker\_coins\_given = joker\_coins\_total / 3 
     \indent \#The answer is 
     \indent result = joker\_coins\_given 
     \indent return result

==> sections/old_intro.tex <==
% Paragraph 1: Motivation. What's the problem and why is it important?
% - Focus on the model: Need more test-prep questions, LLMs have been used to generate lots of high-quality data but not for test-prep. There's lots of math LLMs now and so we aim to develop math LLMs to generate test-prep questions.
% Paragraph 2: State-of-the-art and what's missing (most LLMs are answers, not question generators)
% Paragraph 3: Specifically what do we want to do? "We aim to train a question--generator..."
% Paragraph 4: Why is this hard/what's the limitation?
% Paragraph 5: What do we propose in this work and what do we find?
% Paragraph 6: Contributions (bullet-point list, 1 sentence per contribution---go look at examples!)
Math word problems are critical for assessing learning in K-12 education \cite{daroczy_word_2015, article, schwartz_why_2023,verschaffel_word_2020}. Customizing word problems to student interests can increase learning, interest in math, and test performance \cite{bernacki_role_2018, walkington_using_2013, walkington_personalizing_2019}. However, with severe time constraints, teachers can rarely customize questions.
Given rapid recent progress in math reasoning, we propose that language models stand to bolster math education by generating customized, diverse math word problems for students.
However, the capacity of language models to generate \textit{educational} problems remains unstudied.
% burdens by automatically generating  exciting opportunity to accelerate question generation, 
% We aim to automatically generate customized math word problems and answers to promote interest-guided math education.

\begin{table*}[t]
    \centering 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{p{.1\linewidth}p{.6\linewidth}p{.3\linewidth}} \toprule
         \textbf{Dataset}& \textbf{Example} &\textbf{Educational Appropriateness} \\ \midrule
         GSM8K&  Henry took 9 pills a day for 14 days. Of these 9 pills, 4 pills cost \$1.50 each, and the other pills each cost \$5.50 more. How much did he spend in total on the pills? \newline
         & \xmark \hspace{.25cm}This question mentions taking pills, which is not appropriate for young learners.\\
          EGSM$_\text{Train}$ (Ours)&  Barbie has 100 pink outfits. She has 20 more blue outfits than pink outfits. She has 50\% more green outfits than blue outfits. How many outfits does Barbie have in total?& $\checkmark$ \\ \bottomrule
    \end{tabular}}
    \caption{Example from both GSM8K and EGSM$_\text{Train}$ (ours). EGSM$_\text{Train}$ is the only teacher validated grade school math dataset, while existing datasets contain problems inappropriate for young learners.}
\label{dataset_comparison}
\end{table*}
    \label{tab:example_problem_comparison}
%Systems that generate large volumes of appropriate math problems could accelerate problem customization, improving math education.
% We aim to leverage recent advances in large language models (LLMs) \cite{brown_language_2020} to efficiently automatically generate customized math word problems and answers.
% With the recent proliferation of large language models (LLMs) \cite{brown_language_2020}, it is possible for teachers to use these models to automatically generate customized word problems and answers.
\input{sections/generation_process}

Math word problems are natural language questions paired with numerical solutions, as illustrated in Figure \ref{fig:mathwell_example}. To be effective educational tools for grade-school students, the problems must be solvable, appropriate, and have accurate solutions.
While most public word problem resources are manually curated and limited (e.g., \citealt{noauthor_free_nodate, noauthor_teaching_nodate, noauthor_sol_nodate}), there have been recent efforts to generate these problems using natural language processing \cite{jiao_automatic_2023, koncel-kedziorski-etal-2016-theme, niyarepola_math_2022, norberg2023rewriting, qin_mathematical_2023, qin_math_2024, wang_math_2021, wu_automatic_2022,zhou_towards_2019, zhou2023learning, zong_solving_2023}.
% The traditional approach to automatically generating math word problems is to use deep neural networks to generate problems based on pre-specified equations and/or reference problems \cite{jiao_automatic_2023, koncel-kedziorski-etal-2016-theme, norberg2023rewriting, qin_mathematical_2023, wang_math_2021, zhou_towards_2019, zhou2023learning}.
Closest to our work, some recent efforts have begun exploring math word problem generation using Large Language Models (LLMs) \cite{niyarepola_math_2022,zong_solving_2023}.

However, to the best of our knowledge, existing methods have one or both of two important limitations.
First, many only generate questions (e.g., \citealt{niyarepola_math_2022, zong_solving_2023}).
To be educationally useful, students and teachers must also have access to answers.
Further, it is hard to verify if questions are solvable and appropriate without answers.
Second, all existing methods are \textit{reference-dependent}, simply rephrasing or creating new output based on input problems or equations.
In practice, curating and choosing specific word problems or equations beforehand is laborious and difficult \cite{roche2013choosing}, and there are more equations and word problem templates than can reasonably be pre-specified. A more flexible approach to word problem generation can ensure students master different types of word problems rather than memorize operations associated with specific phrasing/template equations, which harms generalizability and limits overall learning  \cite{ben-zeev_spurious_2001, chang_learning_2003}. 

To address the aforementioned limitations, we propose \textit{reference-free} educational math word problem generation.%There are also contexts for which having increased flexibility over question structure and underlying equations may be preferable, such as preparing students for problems that mix/combine operations or allowing students to practice solving problems on their own without knowing the equation the problems will follow before generation. 
Successful solutions must return questions and answers together and require no hand-picked equations or exemplar word problems. 
For reference-free word problem generators to be useful educational tools, we propose three criteria to evaluate their outputs.
1) Each problem must be \textit{solvable}.
2) Each question's corresponding answer must be \textit{accurate}.
3) Each problem must be \textit{appropriate}, where the question/answer must make logical sense, the math topic must be familiar to a student, and the question's content must be appropriate for a young learner. \newline \indent To explore reference-free appropriate, educational math word problem generation, we introduce MATHWELL, the first such generator trained through finetuning Llama-2 (70B) in two stages. The first stage uses popular math question-answering (QA) datasets used in recent work \cite{azerbayev_llemma_2023, luo2023wizardmath, yue_mammoth_2023}. However, these datasets are not designed to train word problem generators and teachers find that they are educationally inappropriate, which we show qualitatively in Figure \ref{tab:example_problem_comparison} and quantitatively in Figure \ref{fig:barplot}. In turn, we use our first-stage model to generate the first dataset designed to train educational word problem generators and the only grade school math dataset annotated by teachers. To demonstrate the data's quality and improve our model, we use it to conduct a second stage of finetuning. We show MATHWELL's outputs are better targeted for grade school math education than those from existing open and closed source alternatives. While our model generates word problems without the need for a reference problem or equation, we show that its outputs are non-trivially controllable in Table \ref{main_results} and Appendix \ref{controllability_experiment}. Specifically, without exploring prompt engineering or additional training, we are able to control the math operations present in MATHWELL generations at a rate that is competitive with the rate at which existing SOTA word problem generators successfully incorporate a pre-specified equation.
%OLD
%We propose Math Assessment Through High-interest Word Problems Extracted from LLMs (MATHWELL), the first reference-free educational math word problem generator.
%MATHWELL is a Llama-2 (70B) model finetuned on popular math question-answering (QA) datasets used by recent math LLMs \cite{azerbayev_llemma_2023, luo2023wizardmath, yue_mammoth_2023}.
%However, these datasets are unannotated for solvability, accuracy, and appropriateness and are not designed to train word problem generators.
%We therefore conduct multiple rounds of annotation by real expert educators, which we use to progressively finetune MATHWELL.
%With these annotations, our resultant model's outputs are better targeted for grade-school math education than outputs from alternative general-purpose math LLMs.
%Further, we train MATHWELL to generate Program of Thought (PoT) solutions to word problems, which recent methods show improves accuracy on open-ended questions \cite{azerbayev_llemma_2023, gao_pal_2023, yue_mammoth_2023}.


% Old paragraph
% Existing grade school math datasets are intended for training math question-answering (QA) models rather than question generators \cite{cobbe_training_2021, gao_pal_2023, miao_diverse_2020, mishra_numglue_2022, patel_are_2021}. In turn, none of these datasets are aligned with the criteria we find necessary for training reference-free word problem generators. Additionally, generated questions must be solvable, have accurate solutions, and be appropriate for young learners with respect to mathematical difficulty and content discussed, each of which are nontrivial tasks and are different objectives than those typically used to train LLMs. 

% OLD METHODS PARAGRAPH
% We propose a reference-free word problem generator, Mathematics Assessment Through High-interest Word Problems Extracted from LLMs (MATHWELL), that generates a question/answer pair aligned with an optional student interest. To create this model, we first finetune Llama-2 (70B) \cite{touvron2023llama} on existing math QA data with Python code solutions. Next, we generate synthetic data from this model that have solutions in the form of Python functions and have experts annotate that data based on our three proposed evaluation metrics of solvability, accuracy and appropriateness to identify high-quality generations. Finally, we further finetune our model on the high-quality generations to create MATHWELL. 

%We use MATHWELL to generate Educational Grade School Math (EGSM), containing 20,490 word problems.
%This is the largest public set of English math word problems with PoT rationales.
We use MATHWELL to generate Educational Grade School Math (EGSM), containing 20,490 word problems. We acquire annotations from domain experts for 3,484 MATHWELL outputs during and after training to score the quality of our data, resulting in a EGSM$_\text{Train}$ subset with 2,093 samples with gold labels for solvability, accuracy, and appropriateness.
We find that MATHWELL is effective at generating custom math word problems without reference problems or equations: 74\% of its output problems with executable code are simultaneously solvable, accurate, and appropriate and nearly all successfully include a specified topic. MATHWELL has a nearly 20\% higher share of outputs with executable code that meet our three evaluation criteria than existing open-source LLMs, outperforming GPT-3.5 Turbo and matching 94.9\% of GPT-4 Turbo's performance while also generating problems with a more appropriate reading level and that avoid the most harmful types of inappropriate questions.
%outputs with executable code are nearly 20\% more likely to meet our three evaluation criteria than alternative LLMs.
%Further, we find that EGSM is more age appropriate in terms of readability than other datasets.
Further, we find that EGSM has a more appropriate reading level than other datasets.
% Preliminary experiments show our human annotations can be used to train text classifiers to automatically evaluate outputs from reference-free word problem generators, especially along the dimensions of appropriateness and solvability. 

% OLD PARAGRAPH
% We find that MATHWELL is effective at generating math word problems without context: 76\% of its question/answer pairs with executable code identified as meeting our evaluation criteria, but also data generated from this model is of high quality for training reference-free word problem generators and is comparable to human-written math QA datasets. Preliminary experiments show our human annotations can be used to train text classifiers to automatically evaluate outputs from reference-free word problem generators, especially along the dimensions of appropriateness and solvability. 

Our work has the following contributions: 
\begin{itemize}
    \item We introduce a novel reference-free word problem generation task and, through expert human annotation, propose solvability, accuracy and appropriateness as the primary metrics for evaluating output from these models.
    \item Using these criteria, we conduct evaluations that show existing datasets fail to be educationally appropriate. 
    \item We curate and release EGSM, the first dataset designed to train educational reference-free grade school math word problem generators.
    \item     We further evaluate EGSM$_\text{Train}$, the only teacher annotated grade school math dataset, by using it to finetune MATHWELL, which has a 43.4\% higher share of outputs that meet all three criteria and have executable code than the next best open-source model and nearly eliminates the gap between open and closed source models on this task. MATHWELL is the only model that consistently outputs questions at an appropriate reading level for K-8 students and avoids the most harmful types of inappropriate content for young learners. %MATHWELL's performance despite being trained solely through finetuning demonstrates the value of our data.
    
\end{itemize}

==> sections/unedited_auto_eval_table.tex <==
\begin{table*}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
\textbf{Source}& \textbf{PPL $\downarrow$} & \textbf{M PPL $\downarrow$}& \textbf{BF1}& \textbf{M BF1}& \textbf{A/M BF1}&\textbf{G BF1} & \textbf{AL}&\textbf{M AL} &\textbf{NDC}\\
\midrule
 MathInstruct GSM8K& 3.07 (0.691)&--& 84.6& --& --&-- & \textbf{65.7* (23.7)}&-- &8.15 (1.12)\\
 SGSM Train& 2.44 (0.439)&--& 85.2& --& --&84.4 & 57.3 (15.7)&-- &8.13 (1.25)\\
 SGSM Unannotated& \textbf{2.33 (0.679)}& --& 84.9& --& --&84.0& 62.2 (14.9) &-- &7.98 (1.28)\\
LLEMMA& 3.79 (1.60)& 3.12 (0.615)& 84.3& 85.3& 84.6&84.4 & 56.5 (1.43)&52.5 (2.60)&8.48 (1.19)\\
MAmmoTH& 2.75 (0.526)& 2.74 (0.517)& 85.9& 86.4& 86.1&84.8 & 46.1 (1.13)&44.04 (1.16)&8.27 (1.24)\\
 Llama-2& 2.48 (0.527)& 2.47 (0.512)& 85.4& 85.8& 85.6&84.5& 53.1 (0.991&51.57 (1.16)&8.24 (1.15)\\
MATHWELL& 2.45 (0.439)& \textbf{2.46 (0.427)}& 85.6& 85.7& 85.6&84.3& 55.2 (0.878)&\textbf{54.4 (1.01)}&8.31 (1.27)\\
\bottomrule
\end{tabular}
}
\caption{\label{citation-guide}Automatic evaluation metrics for each training dataset or model. BF1 is BERTScore F1, M is MaC, A/M BF1 compares all to MaC questions, G BF1 compares each source's questions to MathInstruct GSM8K, and AL is average token length. Bold indicates the lowest PPL and longest AL in each column. A * indicates the difference between the longest AL and the second longest AL is statistically significant at the p<.01 level. A -- in dataset rows indicates the dataset is either fully MaC (MathInstruct GSM8K/SGSM Train) or does not have a MaC subset (SGSM Unannotated). Standard deviations, where applicable, are in parentheses.
}
\label{tab:auto_eval}
\end{table*}

==> sections/unedited_table_2.tex <==
\begin{table*}[t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccclcccc}
\toprule
\textbf{Dataset}& \textbf{N}& \textbf{PoT}&\textbf{PF}&\textbf{AD} &\textbf{TA}& \textbf{AL}&\textbf{FKGL} &\textbf{NDC}&\textbf{BF1}\\ 
\midrule
 GSM-Hard& 1,319&  $\checkmark$&  $\checkmark$& \xmark  &\xmark& 72.9 (25.6)&4.21 (2.43)&8.20 (1.13)&84.0\\
 GSM8K& 8,792& \xmark& \xmark& $\checkmark$  & \xmark& 67.0 (24.4)& 4.24 (2.47)& 8.19 (1.13)&84.5\\
MathInstruct GSM8K& 6,403&   $\checkmark$&  \xmark&  $\checkmark$  &\xmark& 66.2 (23.9)&4.25 (2.48)&8.17 (1.13)&84.6\\
%NumGLUE \cite{mishra_lila_2022}& 12,403&  $\checkmark$ & \xmark & \xmark & 144.8 (136.5)&10.04 (6.99)&10.27 (1.51)&81.5\\
ASDIV& 2,305&  \xmark&  \xmark&  $\checkmark$  &\xmark& 45.1 (15.8)&3.56 (2.40)&7.85 (1.48)&85.5\\
 SVAMP& 1,000& \xmark& \xmark& $\checkmark$  &\xmark& 47.3 (11.7)& 3.39 (2.07)& 7.84 (1.09)&86.1\\
 EGSM (Ours) & 20,490& $\checkmark$& $\checkmark$& ? &\xmark& 62.0 (15.0)& 2.68 (1.97)& 7.99 (1.26)&84.8\\
 \hspace{3mm}EGSM$_\text{Train}$& 2,093& $\checkmark$& $\checkmark$& $\checkmark$  &$\checkmark$  & 57.2 (15.7)& 2.50 (1.76)& 8.12 (1.25)&85.2\\
 \hspace{3mm}EGSM$_\text{Unannotated}$& 18,397& $\checkmark$& $\checkmark$& ? &\xmark& 62.5 (14.8)&2.70 (1.99)&7.97 (1.26)&84.9\\
 \bottomrule
\end{tabular}
}
\caption{\label{citation-guide}Characteristics of datasets with more than 1,000 examples that can be used to train reference-free word problem generators. N is the deduplicated number of questions, PF is Python function solution, AD is appropriate difficulty, TA is teacher annotated, AL is average length (in tokens), FKGL is Flesch-Kincaid grade level, NDC is New Dale-Chall readability, and BF1 is BERTScore F1. A ``?'' denotes we cannot verify whether all questions are written at an appropriate difficulty due to the dataset being unannotated. Standard deviations, where applicable, are in parentheses.}
\label{unedited_tab_2}
\end{table*}

\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{clccccc}
\toprule
& \textbf{Model}& \textbf{PPL $\downarrow$} & \textbf{BF1}&\textbf{GSM BF1}&\textbf{MaC AL}&\textbf{NDC}\\ \midrule
 % Closed-source Models& & & & &\\
\parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{API}}} &
GPT-4 Turbo& 2.50 (0.03)& 85.4& 84.6& 66.8 (2.62)&8.26 (0.07)\\
& GPT-3.5 Turbo& 2.64 (0.03)& 85.6& 84.6& 49.9 (1.16)&8.58 (0.07)\\
\midrule
 % Open-source Models& & & & &\\
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Public}}} &
LLEMMA& 3.82 (0.10)& 84.3&84.0&50.9 (2.89)&8.41 (0.09)\\
& MAmmoTH& 2.76 (0.03)& 86.0&84.6&44.4 (1.15)&8.25 (0.08)\\
 & Llama-2& 2.52 (0.03)& 85.5&84.3&49.8 (1.19)&8.20 (0.07)\\
& MATHWELL& \textbf{2.44 (0.03)}& 85.5&84.2&\textbf{54.1 (0.97)}&8.23 (0.08)\\
\bottomrule
\end{tabular}
}
\caption{\label{citation-guide}Automatic evaluation metrics for each model. PPL is perplexity, BF1 is BERTScore F1, GSM BF1 compares each model's questions to GSM8K, MaC is meets all criteria, AL is average token length, and NDC is New Dale-Chall readability. Bold indicates the lowest PPL and longest AL for MaC generations for open-source models. Standard errors, where applicable, are in parentheses.
}
\label{tab:auto_eval_models}
\end{table}

==> tables/big_table.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{3.7pt}     % slight adjustment to fit text width
\setlength{\cmidrulekern}{0.25em}
\resizebox{\linewidth}{!}{
\begin{tabular}{l*{13}{c}}
\toprule
 & \multicolumn{4}{c}{\textbf{zsRE} (T5; F1 $\uparrow$)} & \multicolumn{4}{c}{\textbf{SCOTUS} (BERT; Acc $\uparrow$)}  & \multicolumn{5}{c}{\textbf{Hallucination} (GPT2-XL; PPL $\downarrow$)} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-14}
\textbf{Method} & TRR & ERR & \textit{Avg.} & \textit{\#E} & TRR & ERR & \textit{Avg.} & \textit{\#E} & TRR & ERR & ARR & \textit{\#E} & time (s)\\
\midrule
FT \cite{lin2022continual}              & .56 & .82 & \textit{.69} & 1000 & .52 & .52 & \textit{.52} & 415 & 1449.3 & 28.14 & 107.76 & 1392 & .26 (.07)\\
FT+EWC \cite{kirkpatrick2017overcoming} & .51 & .82 & \textit{.66} & 1000 & .67 & .50 & \textit{.58} & 408 & 1485.7 & 29.24 & 109.59 & 1392 & .29 (.06)\\
FT+Retrain \cite{rolnick2019experience} & .27 & .99 & \textit{.63} & 1000 & .67 & \textbf{.83} & \textit{.75} & 403 & 2394.3 & 35.34 & 195.82 & 1392 & 23.4 (13.2)\\
MEND \cite{mitchell2021fast}            & .25 & .27 & \textit{.26} & 1000 & .19 & .27 & \textit{.23} & 672 & 1369.8 & 1754.9 & 2902.5 & 1392 & .63 (.10) \\
Defer \cite{mitchell2022memory}          & \textbf{.72} & .31 & \textit{.52} & 1000 & .33 & .41 & \textit{.37} & 506 & 8183.7 & 133.3 & 10.04 & 1392 & .07 (.02) \\
ROME \cite{meng2022locating}            & --- & --- & --- & --- & --- & --- & --- & --- & 30.28 & 103.82 & 14.02 & 1392 & \ .64 (.28)\\
Memory                                  & .25 & .27 & \textit{.26} & 1000 & .21 & .20 & \textit{.21} & 780 & 25.47 & 79.30 & 10.07 & 1392 & .11 (.02) \\
GRACE & .69 & \textbf{.96} & \textbf{\textit{.82}} & 1000 & \textbf{.81} & .82 & \textbf{\textit{.82}} & 381 & \textbf{15.84} & \textbf{7.14} & \textbf{10.00} & 1392 & .13 (.02)\\
\bottomrule
\end{tabular}
}
\caption{My table.}\label{tab:main_results}
\end{table*}


==> tables/original_math_ops.tex <==
\begin{tabular}{lccccccc}
\toprule
\textbf{Model}& \textbf{Add. (\%)}& \textbf{Sub. (\%)}& \textbf{Mult. (\%)}& \textbf{Div. (\%)}& \textbf{Frac. (\%)}&\textbf{Dec. (\%)}&\textbf{No Ops (\%)}\\
\midrule
LLEMMA& 36.3& 31.5& 33.1& 19.4& 5.6& 14.5&14.5\\
MAmmoTH& 39.4& 37.6& 43.6& 19.7& 3.7& 10.6&2.3\\
 Llama-2& 59.6& 57.7& 23.5& 11.7& 8.0& 10.3&5.2\\
MATHWELL& 69.5& 66.4& 22.0& 12.6& 4.9& 7.6&1.3\\
\bottomrule\\
\end{tabular}
}

MaC Questions:
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule
\textbf{Model}& \textbf{Add.}& \textbf{Sub.}& \textbf{Mult.}& \textbf{Div.}& \textbf{Frac.}&\textbf{Dec.}&\textbf{Total Ops}\\
\midrule
LLEMMA& 39.0& 43.9& 31.7& 14.6& 2.4& 12.2&1.4\\
MAmmoTH& 42.1& 41.4& 41.4& 17.1& 5.0& 10.0&1.6\\
 Llama-2& 64.3& 59.9& 25.5& 10.2& 5.1& 7.6&1.7\\
MATHWELL& 70.7& 67.0& 21.8& 12.2& 4.8& 6.9&1.8\\
\bottomrule
\end{tabular}
}
\caption{\label{citation-guide}Characteristics of model-generated questions. All columns are percentages, except total ops, which reports the average total operations in each question.
}
\label{operations}
\end{table*}
